Agentic Delegation and the Language Frontier of Software Developers: A Model and Evidence from Claude Code on GitHub

We develop and test a model of agentic delegation in software production. Developers face language-specific entry thresholds; conversational AI mainly augments work in languages they already know, while agentic AI adds delegated execution under developer specification and verification. The model predicts an activation band of unfamiliar languages that become feasible only with an agent, expanding the observed language-production frontier of the developer. We test this prediction in a monthly GitHub panel of 5,346 developers, dating adoption by first Claude Code co-authorship and constructing commit-level language outcomes from 57 million changed files. Doubly robust staggered-adoption event studies with not-yet-treated comparisons show sharp expansion at adoption: active languages rise by 2.5 relative to a 0.9 baseline, newly used languages by 1.2, entropy by 0.38, and cumulative breadth continues to grow afterward. The pattern survives removing the treatment-defining language, excluding all Claude-coauthored commits, conditioning on activity, and screening users of competing agents. Consistent with the model, first uses of unfamiliar languages concentrate among narrow pre-adoption specialists at each activity level. Because adoption is voluntary and may coincide with project shocks, the estimates are event-time associations rather than definitive causal effects.

==> tables/table01_summary_stats.tex <==
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{Treated} & \multicolumn{1}{c}{Control} & \\
\cmidrule(lr){2-3}\cmidrule(lr){4-4}
Variable & Pre-adoption & Post-adoption & All months & Diff. (Post $-$ Control) \\
\midrule
Monthly commits & 16.05 & 46.69 & 19.09 & 27.60 \\
 & (129.79) & (152.43) & (96.69) & \\
Repositories & 1.02 & 2.07 & 1.02 & 1.05 \\
 & (2.55) & (3.99) & (2.63) & \\
Programming languages & 0.60 & 1.16 & 0.59 & 0.57 \\
 & (1.02) & (1.33) & (1.01) & \\
Language entropy (Shannon) & 0.09 & 0.18 & 0.09 & 0.10 \\
 & (0.25) & (0.33) & (0.24) & \\
Newly-used languages & 0.16 & 0.17 & 0.14 & 0.03 \\
 & (0.47) & (0.46) & (0.44) & \\
Cumulative languages & 1.64 & 4.07 & 1.90 & 2.17 \\
 & (2.04) & (2.63) & (2.24) & \\
\midrule
Developers & \multicolumn{2}{c}{3,060} & 2,778 & \\
Months & \multicolumn{4}{c}{28} \\
Observations (panel rows) & \multicolumn{4}{c}{163,464} \\
\bottomrule
\end{tabular}

==> tables/table02_main_results.tex <==
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{3}{c}{Event-time ATT} & \\
\cmidrule(lr){2-4}
Outcome & $t=0$ & $t=1$ & $t=2$ & Simple ATT \\
\midrule
Monthly commits & $40.708^{*}$ & $24.004$ & $13.277$ & $20.822^{*}$ \\
 & $(2.674)$ &  &  & $(2.738)$ \\
Repositories & $1.497^{*}$ & $0.804$ & $0.422$ & $0.717^{*}$ \\
 & $(0.059)$ &  &  & $(0.054)$ \\
Programming languages & $0.830^{*}$ & $0.392$ & $0.210$ & $0.360^{*}$ \\
 & $(0.020)$ &  &  & $(0.021)$ \\
Language entropy & $0.138^{*}$ & $0.072$ & $0.041$ & $0.067^{*}$ \\
 & $(0.006)$ &  &  & $(0.006)$ \\
Newly-used languages & $0.308^{*}$ & $-0.019$ & $-0.053$ & $0.035^{*}$ \\
 & $(0.014)$ &  &  & $(0.011)$ \\
Cumulative languages & $0.507^{*}$ & $0.565$ & $0.610$ & $0.586^{*}$ \\
 & $(0.016)$ &  &  & $(0.022)$ \\
\midrule
Developers & \multicolumn{4}{c}{5,838\;(\;3,060\;treated,\;2,778\;control)} \\
\bottomrule
\end{tabular}

==> tables/table03_robustness.tex <==
\begin{tabular}{lccc}
\toprule
 & \multicolumn{3}{c}{ATT at $t=0$ by sample restriction} \\
\cmidrule(lr){2-4}
Outcome & Main & $\geq50\%$ pre-active & $\geq6$ pre-months \\
\midrule
Monthly commits & $40.708^{*}$ & $43.616^{*}$ & $38.974^{*}$ \\
 & $(2.674)$ & $(5.668)$ & $(3.863)$ \\
Repositories & $1.497^{*}$ & $1.634^{*}$ & $1.538^{*}$ \\
 & $(0.059)$ & $(0.150)$ & $(0.096)$ \\
Programming languages & $0.830^{*}$ & $0.623^{*}$ & $0.710^{*}$ \\
 & $(0.020)$ & $(0.044)$ & $(0.035)$ \\
Language entropy & $0.138^{*}$ & $0.121^{*}$ & $0.140^{*}$ \\
 & $(0.006)$ & $(0.013)$ & $(0.011)$ \\
Newly-used languages & $0.308^{*}$ & $0.173^{*}$ & $0.220^{*}$ \\
 & $(0.014)$ & $(0.021)$ & $(0.018)$ \\
Cumulative languages & $0.507^{*}$ & $0.203^{*}$ & $0.234^{*}$ \\
 & $(0.016)$ & $(0.025)$ & $(0.020)$ \\
\midrule
Developers ($N$) & 5,838 & 1,620 & 2,672 \\
\bottomrule
\end{tabular}

==> tables/table_cl_comparison.tex <==
\begin{tabular}{lcc}
\toprule
 & \multicolumn{2}{c}{ATT at adoption ($t=0$)} \\
\cmidrule(lr){2-3}
Outcome & Repository-level & Commit-level \\
\midrule
Programming languages & $0.830^{*}$ & $2.528^{*}$ \\
 & $(0.020)$ & $(0.063)$ \\
Language entropy & $0.138^{*}$ & $0.382^{*}$ \\
 & $(0.006)$ & $(0.009)$ \\
Newly-used languages & $0.308^{*}$ & $1.193^{*}$ \\
 & $(0.014)$ & $(0.051)$ \\
Cumulative languages & $0.507^{*}$ & $1.604^{*}$ \\
 & $(0.016)$ & $(0.054)$ \\
\midrule
Language measure & repo primary language & every changed file (Linguist) \\
\bottomrule
\end{tabular}
